Monitoring of Perception Systems: Deterministic, Probabilistic, and Learning-based Fault Detection and Identification

This paper investigates runtime monitoring of perception systems. Perception is a critical component of high-integrity applications of robotics and autonomous systems, such as self-driving cars. In these applications, failure of perception systems may put human life at risk, and a broad adoption of these technologies requires the development of methodologies to guarantee and monitor safe operation. Despite the paramount importance of perception, currently there is no formal approach for system-level perception monitoring. In this paper, we formalize the problem of runtime fault detection and identification in perception systems and present a framework to model diagnostic information using a diagnostic graph. We then provide a set of deterministic, probabilistic, and learning-based algorithms that use diagnostic graphs to perform fault detection and identification. Moreover, we investigate fundamental limits and provide deterministic and probabilistic guarantees on the fault detection and identification results. We conclude the paper with an extensive experimental evaluation, which recreates several realistic failure modes in the LGSVL open-source autonomous driving simulator, and applies the proposed system monitors to a state-of-the-art autonomous driving software stack (Baidu's Apollo Auto). The results show that the proposed system monitors outperform baselines, have the potential of preventing accidents in realistic autonomous driving scenarios, and incur a negligible computational overhead.

==> includes/redeclare_utils.tex <==
\makeatletter
\newcommand\RedeclareMathOperator{%
  \@ifstar{\def\rmo@s{m}\rmo@redeclare}{\def\rmo@s{o}\rmo@redeclare}%
}
% this is taken from \renew@command
\newcommand\rmo@redeclare[2]{%
  \begingroup \escapechar\m@ne\xdef\@gtempa{{\string#1}}\endgroup
  \expandafter\@ifundefined\@gtempa
     {\@latex@error{\noexpand#1undefined}\@ehc}%
     \relax
  \expandafter\rmo@declmathop\rmo@s{#1}{#2}}
% This is just \@declmathop without \@ifdefinable
\newcommand\rmo@declmathop[3]{%
  \DeclareRobustCommand{#2}{\qopname\newmcodes@#1{#3}}%
}
\@onlypreamble\RedeclareMathOperator
\makeatother


==> sections/subsections/ablation_GNN.tex <==
\subsubsection{Ablation Study on GNN Node Features}\label{sec:ablation_study_features}

We provide additional ablation studies for fault identification using GNNs.
In particular we tested the networks with the same parameters but different features nodes.

In the first test we changed how the test node features are computed.
Let $\test_k$ be a \dtest comparing two obstacles set $\lobs$ and $\robs$.
Each obstacle in each set might have a confidence associated representing how confident is the module that produced it.
Let $c_\lobs$ and $c_\robs$ be the minimum confidence over the set of obstacles $\lobs$ and $\robs$, respectively.
% We can interpret the confidence of an obstacle, as the probability of the correctness of the obstacle information.
% Even if this interpretation is not entirely correct, it is still a useful way to use the confidence of an obstacle to compute the feature vector.
We then take the confidence of a test as $c_{\test_k} =\min(c_\lobs,c_\robs)$.
Whenever the confidence of the output is not available, we assume it is $1$.
The feature of test variables is then the one-hot encoding of the test outcome, weighed by the test confidence, formally $\vxx_{\test_k} = c_{\test_k}\onehot(\syndromevar_{\test_k})$.

\input{tables/fault_identification_alt_tests.tex}

\red{
In the second test we changed the features of the \fmodes.
For a feature vector $\vxx_{\failure_i}\in\Reals{2}$ of a \fmode $\failure_i$ we take $\vxx_{\failure_i}=[j, i]\tran$ where $j$ is a unique integer representing unit (module or output) that can experience that failure mode.

\input{tables/fault_identification_alt_fmodes.tex}

The different feature choices do not substantially improve the fault identification performance.

With the choice of confidence-weighted one-hot encoding of the test outcomes, GCN and GIN attain worse performances with regular \dgraphs while GCNII and GraphSage exhibit an improvement.
However, when using temporal \dgraphs all the architectures have worse performance except for GCNII.
GNCII is the architecture that is able to exploit the feature the best, which suggest that confidence-weighted one-hot encoding of the test outcomes should be used in combination with GCNII.

With the change in the \fmodes features, all architectures seem to work better in with the regular \dgraphs (excluding GNC that worsen), but the performance in the temporal \dgraphs steeply decrease.

\input{tables/fault_identification_alt_both.tex}

}

==> sections/subsections/diagnosability.tex <==
%!TEX root = ../../main.tex



==> sections/subsections/discarded.tex <==
%!TEX root = ../../main.tex
% In particular, we distinguish \emph{test-driven relations} 
% $\rel_k(\faults})\in\relset = \rel_k(\faults_{\scope(\test_k)}; \syndromevar_k)$

% $\rel_k(\faults)\in\relset$

% $\rel_k(\faults})\in\relset = \rel_k(\faults_{\scope(\test_k)}; \syndromevar_k)$
% $\rel_k(\faults_{\scope(\test_k)}; \syndromevar_k)\in\relset$ in $\relset$, if $\failure_i$ is in the scope of the \relation $\rel_k$.



\grayout{


  A \dgraph can encode deterministic or probabilistic information.
The difference between the two is only in the codomain of the \relations.
In the deterministic case, a \relation encodes the set of possible assignments given the syndrome $\syndrome$, $\rel:\powerset(\varset)\times\{\mathpass, \mathfail\}^{\nrtests}\to\{\ltrue,\lfalse\}$, it returns $\ltrue$ is the assignment is feasible, $\lfalse$ otherwise.
The relation for a test $\test$ will take the form
\begin{equation}
  \rel(\faults;\syndrome) = \begin{cases}
    \ltrue & \text{if } \exists \faults \;:\; \syndromevar_\test = \test\left(\faultsover{\scope(\test)}\right) \\
    \lfalse & \text{otherwise}
  \end{cases}
\end{equation}
For example, for the OR test in~\cref{tab:tfactor_1} we would have
\begin{equation*}
  \rel(\faults;\syndrome) = \begin{cases}
    \lfalse & \text{if } \syndromevar_\test + \failure_1 + \failure_2 = 1 \\
    \ltrue & \text{otherwise} 
  \end{cases}
\end{equation*}



\subsection{Examples of \DTests}

Consider the simple example in figure \cref{fig:simple_dgraph}.
In this \dgraph~there are three \fmodes~($\failure_1$, $\failure_2$ and $\failure_3$) and two \dtests~($\test_1$ and $\test_2$) whose test outcomes are represented by $\syndromevar_1$ and $\syndromevar_2$.
We can consider each \fmode~to be associated with different outputs in the system, while the \modules~that generated the outputs do not have any \fmode~associated with them.
We say that $\scope(\test_1) = \{\failure_1,\failure_2\}$ and similarly $\scope(\test_2) = \{\failure_2, \failure_3\}$.
The factors $\tfactor_i$ $i=1,2$ represent the relationship that there is between the outcome of test $\test_i$ (namely, $\syndromevar_i$) and the state of the \fmodes~in the test's scope.
In discrete factor graphs, we can represent these relationships using tables of potentials.
In this paper, we identify deterministic and probabilistic \dtests.

% \begin{figure}[htbp]
%   \centering
%   \includestandalone{figures/simple_dgraph}
%   \caption{Simple Example of \DGraph}
%   \label{fig:dg_three2}
% \end{figure}

\myParagraph{Deterministic}
In the deterministic \dtests, the tables with potential will contain only $1$ and $0$ values.
Suppose the tests are perfect~\cref{sec:dtests}.
The potentials for factor $\tfactor_1$ in \cref{fig:simple_dgraph} are reported in the column `Perfect test' in \cref{tab:tfactor_1} (the table for $\tfactor_2$ would change only in the name of the columns).
In the table, a value of $1$ in the last column means `possible' while $0$ means `impossible'. 
For example, if we take the first row, it says that if $\failure_1$ and $\failure_2$ are not \factive, it is possible for $\test_1$ to return $0$ outcome.
Conversely, in the fifth row, it says that it not possible for $\test_1$ to return \fail~($1$) if both \fmodes~in its scope are \finactive.
For example suppose that $\test_1$ fails, $\tfactor_1$ says that the possible states for $(\failure_1, \failure_2)$ are $(0,1)$, $(1,0)$ and $(1,1)$.
Similarly, $\tfactor_2$ says that the possible states for $(\failure_2, \failure_3)$ are $(0,0)$, $(1,1)$.
Joining the possible states we get that the possible states for $(\failure_1, \failure_2, \failure_3)$ are $(0,1,1)$, $(1,0,0)$, $(1,1,1)$.
Without additional information, we cannot say which of the possible states is the correct one.
We will study this phenomenon in~\cref{sec:foundamental_limits}.
}

==> sections/subsections/preliminaries.tex <==
%!TEX root = ../../main.tex



==> sections/subsections/scenarios_heath.tex <==
%!TEX root = ../../main.tex

\section{Experimental evaluation}

Intro to experimental section. Todo's are in \textbf{BOLD}.

\subsection{Experimental setup}

\begin{itemize}
	\item Apollo Auto Autonomous driving platform
	\begin{itemize}
		\item Baidu's Apollo Autonomous driving platform is an open source self-driving vehicle tech platform.
		This high-performance software offers the capabilities in obstacle perception, trajectory planning,
		vehicle control, and vehicle operating system. This allows Apollo to guide a vehicle through complex
		traffic scenarios that include traffic lights, pedestrians, and different lane configurations.
		\item Apollo provides a teleoperation inferface with DreamView integration where users can visualize
		the current output of relevant autonomous driving modules. This feature also offers human-machine
		for users to view hardware status, turn on/off modues, and start the autonomous driving car as well
		as debugging tools, to effectively track module issues. This component of Apollo was used extensively
		to monitor our scenarios in real time.
		\item Throughout this experiment we have used the master version of Apollo.
		\item \textbf{Alternatives (For Pasquale)}
	\end{itemize}
	\item Apollo's Perception System
	\begin{itemize}
		\item The Apollo Auto perception system detects objects by utilizing the 128c LIDAR, Front RADAR, and 
		front-facing camera. The object detection system recieves data from each sensor that is then converted
		into a list of objects. It them uses a configurable sensor fusion algorithm to fuse each object 
		detection into a single estimate. Each individual sensor has a different approach to understanding the
		objects around them. The LIDAR represents each object by its 3d convex hull while the RADAR and camera
		parametrize each object with its 3D bounding box. These objects are then plotted onto a diagnostic graph
		that is then interpretted results in the decision the car ultimatly carrys out.
	\end{itemize}
	\item LGSVL Simulator
	\begin{itemize}
		\item LGSVL Simulator is a simulation platform that is commonly used for autonomous vehicles.
		The platform consists of software tools, simulation software, the network content and plugins that 
		allow for personalization, and the cloud environment which allows for the testing of scenarios. 
		The advantages of simulating a virtual environment are endless. Some benefits include the ability 
		to include one or more ego vehicles or autonomous systems and their sensors, as well as different 
		traffic configurations comprised of many dynamics objects. In addition, the simulation software
		provides a customizable interface with a user's System Under Test, giving the devlopers the ability 
		to perform modular testing, debug and perform integration testing.
	\end{itemize}
	\item Our vehicle
	\begin{itemize}
		\item We are using a 2017 Lincoln MKZ, a four door sedan. This car is fitted with a RADAR, LIDAR (32 channels),
		GPS, IMU, a telephoto camera that is pointed marginally up used solely for traffic light detection, and a 
		front-facing monocular camera that is used for obstacle detection.
	\end{itemize}
	\item \textbf{Our pipeline (for Pasquale)}
\end{itemize}

\subsubsection{\DGraph}

\begin{enumerate}
	\item What are the failure modes
	\item Overview of consistency tests
\end{enumerate}

\subsection{Scenarios}

We designed a set of scenarios that included traffic configurations that would effectively test the perception system
of an autonomous vehicle. These scenarios were created using the LGSVL Simulator Visual Scenario Editor. This tool allows
the user to create scenarios for the LGSVL Simulator by first choosing a map from their library, then placing NPC agents 
that are controlled via waypoints, and finally an ego vehicle, which will be controlled by Apollo Auto autonomous driving
platform.

We will now give an explanation of each scenario in the set with the following information: Map, Number of Ego
Vehicles, Number of NPC Agents, the Motivation, the Scenario Descriptions, and the Conditions if modeled after
a real life scenario.
\begin{enumerate}
	\item Overturned Truck
	\begin{enumerate}
		\item \textbf{Map:} Borregas Ave
		\item \textbf{Number of Ego Vehicles:} 1
		\item \textbf{Number of NPC Agents:} 1
		\item \textbf{Motivation:} This is a real life scenario that included a tesla in Taiwan..
		\item \textbf{Scenario Description:} The ego vehicle is driving down a straight road that is occupied by 
		an overturned truck.
		\item \textbf{Conditions:} 12pm and Sunny
	\end{enumerate}
	\item Stopped Vehicle Curved
	\begin{enumerate}
		\item \textbf{Map:} Borregas Ave
		\item \textbf{Number of Ego Vehicles:} 1
		\item \textbf{Number of NPC Agents:} 2
		\item \textbf{Motivation:} This scenario tests the ego vehicles ability to detect two cars ahead.
		\item \textbf{Scenario Description:} While driving, the car in front of the ego vehicle makes a
		lane change to avoid the stationary car that is in their lane. This leaves the ego vehicle with 
		little to no time to react to this stationary car.
		\item \textbf{Conditions:} Any
	\end{enumerate}
	\todo[inline]{should I add information about the stopped vehicle with the jagged turn?}
	\item Invisible Pedestrian
	\begin{enumerate}
		\item \textbf{Map:} Borregas Ave
		\item \textbf{Number of Ego Vehicles:} 1
		\item \textbf{Number of NPC Agents:} 2
		\item \textbf{Motivation:} This scenario tests the ego vehicles ability to detect pedestrains
		that come from blocked areas.
		\item \textbf{Scenario Description:} While driving through a street that has a truck parked on
		the right side, a pedestrian steps into the road from directly behind the parked truck.
		\item \textbf{Conditions:} Any
	\end{enumerate}
	\item Cut Off Left
	\begin{enumerate}
		\item \textbf{Map:} Borregas Ave
		\item \textbf{Number of Ego Vehicles:} 1
		\item \textbf{Number of NPC Agents:} 1
		\item \textbf{Motivation:} This scenario will test the ego vehicles ability to detect objects
		that are behind it. \emph{This scenario is from the Waymo Videos.}
		\item \textbf{Scenario Description:} While driving in the right lane of a three lane road, an agent
		from the left lane cuts the ego vehicle off.
		\item \textbf{Conditions:} 12pm and Sunny
	\end{enumerate}
	\item Cut Off Right
	\begin{enumerate}
		\item \textbf{Map:} Borregas Ave
		\item \textbf{Number of Ego Vehicles:} 1
		\item \textbf{Number of NPC Agents:} 1
		\item \textbf{Motivation:} This scenario will test the ego vehicles ability to detect objects
		that are behind it. \emph{This scenario is from the Waymo Videos.}
		\item \textbf{Scenario Description:} While driving in the left lane of a two lane road, an agent
		from the right lane cuts the ego vehicle off while turning into a parking lot.
		\item \textbf{Conditions:} 12pm and Sunny
	\end{enumerate}
	\item School Bus Intersection
	\begin{enumerate}
		\item \textbf{Map:} Borregas Ave
		\item \textbf{Number of Ego Vehicles:} 1
		\item \textbf{Number of NPC Agents:} 2
		\item \textbf{Motivation:} This scenario is designed to test if the ego vehicle can navigate an
		intersection with two agents.
		\item \textbf{Scenario Description:} The ego vehicle drives through an intersection that includes a
		school bus driving in front of it and a pedestrian walking in front of it.
		\item \textbf{Conditions:} Any
	\end{enumerate}
	\item Cones in the Lane
	\begin{enumerate}
		\item \textbf{Map:} Borregas Ave
		\item \textbf{Number of Ego Vehicles:} 1
		\item \textbf{Number of NPC Agents:} 1
		\item \textbf{Motivation:} This scenario is designed to test if the ego vehicle can detect construction
		objects that are positioned in the lane. \emph{This scenario is from the Waymo Videos.}
		\item \textbf{Scenario Description:} The ego vehicle is traveling straight and there is an agent 
		driving the opposite direction. There are a collection of traffic cones that are positioned in the lane
		that the ego vehicle is driving in.
		\item \textbf{Conditions:} 12pm and Sunny
	\end{enumerate}
	\item Traffic Cones Simple
	\begin{enumerate}
		\item \textbf{Map:} Borregas Ave
		\item \textbf{Number of Ego Vehicles:} 1
		\item \textbf{Number of NPC Agents:} 1
		\item \textbf{Motivation:} This scenario tests in the ego vehicle is capable of detecting the traffic
		cones and that they don't alter the decision making. \emph{This scenario is from the Waymo Videos.}
		\item \textbf{Scenario Description:} The ego vehicle is driving along a road that had traffic cones
		taking up some of the right side. There is an agent driving in the opposite lane.
		\item \textbf{Conditions:} 12pm and Sunny
		\item \textbf{Notes:} This is the same scenario as \emph{Cones in the Lane} except the cones never
		actually enter the ego vehicle's lane, just come very close.
	\end{enumerate}
	\item Traffic Cones Complex
	\begin{enumerate}
		\item \textbf{Map:} Borregas Ave
		\item \textbf{Number of Ego Vehicles:} 1
		\item \textbf{Number of NPC Agents:} 2
		\item \textbf{Motivation:} This scenario tests whether traffic cones will alter the ego vehicle's
		decision making in a more complicated scenario.
		\item \textbf{Scenario Description:} The ego vehicle is driving in a lane with traffic cones to 
		the right while an agent is driving in the opposite direction on the left. After the traffic
		cones have been passed an agent pulls oit of a parkling lot right in front of the ego vehicle.
		\item \textbf{Conditions:} Any
	\end{enumerate}
	\item Cyclist
	\begin{enumerate}
		\item \textbf{Map:} Borregas Ave
		\item \textbf{Number of Ego Vehicles:} 1
		\item \textbf{Number of NPC Agents:} 1
		\item \textbf{Motivation:} This scenario tests if the ego vehicle can detect a cyclist.
		\item \textbf{Scenario Description:} The ego vehicle starts in front of an intersection and once
		it begins driving, a cyclist, from the left side of the intersection, rides right in front of it.
		\item \textbf{Conditions:} Any
	\end{enumerate}
	\item Turkeys
	\begin{enumerate}
		\item \textbf{Map:} GoMentum
		\item \textbf{Number of Ego Vehicles:} 1
		\item \textbf{Number of NPC Agents:} 2
		\item \textbf{Motivation:} This scenario tests the ego vehicle's ability to detect abnormal agents.
		\item \textbf{Scenario Description:} While driving on a straight road, the ego vehicle must avoid
		a collision with two turkeys that walk into the road.
		\item \textbf{Conditions:} Any
	\end{enumerate}
	\item Unprotected Right
	\begin{enumerate}
		\item \textbf{Map:} GoMentum
		\item \textbf{Number of Ego Vehicles:} 1
		\item \textbf{Number of NPC Agents:} 3
		\item \textbf{Motivation:} This scenario tests the ego vehicle's ability to detect cars turning into
		its field of view. \emph{This scenario is from the Waymo Videos.}
		\item \textbf{Scenario Description:} The ego vehicle makes an unprotected right turn on a road that
		contains an agent driving down it as well as another right turn about 20 yards to the left of the 
		ego vehicle that has an agent waiting to exit.
		\item \textbf{Conditions:} Any
	\end{enumerate}
	\todo[inline]{The only information that I didn't include from the notion was \emph{Expected Ego Vehicle
	Behavior} and some of the \emph{Notes}, let me know if this information should be added.}
		
\end{enumerate}

\subsection{Results}

Comment on experiments and results.

==> sections/subsections/tests_example.tex <==
\subsection{Examples of \DTests}

Consider the simple example in figure \cref{fig:simple_dgraph}.
In this \dgraph~there are three \fmodes~($\failure_1$, $\failure_2$ and $\failure_3$) and two \dtests~($\test_1$ and $\test_2$) whose test outcomes are represented by $\syndromevar_1$ and $\syndromevar_2$.
We can consider each \fmode~to be associated with different outputs in the system, while the \modules~that generated the outputs do not have any \fmode~associated with them.
We say that $\scope(\test_1) = \{\failure_1,\failure_2\}$ and similarly $\scope(\test_2) = \{\failure_2, \failure_3\}$.
The factors $\tfactor_i$ $i=1,2$ represent the relationship that there is between the outcome of test $\test_i$ (namely, $\syndromevar_i$) and the state of the \fmodes~in the test's scope.
In discrete factor graphs, we can represent these relationships using tables of potentials.
In this paper, we identify deterministic and probabilistic \dtests.

\begin{figure}[htbp]
  \centering
  \includestandalone{figures/simple_dgraph}
  \caption{Simple Example of \DGraph}
  \label{fig:simple_dgraph}
\end{figure}

\myParagraph{Deterministic}
In the deterministic \dtests, the tables with potential will contain only $1$ and $0$ values.
Suppose the tests are perfect~\cref{sec:dtests}.
The potentials for factor $\tfactor_1$ in \cref{fig:simple_dgraph} are reported in the column `Perfect test' in \cref{tab:tfactor_1} (the table for $\tfactor_2$ would change only in the name of the columns).
In the table, a value of $1$ in the last column means `possible' while $0$ means `impossible'. 
For example, if we take the first row, it says that if $\failure_1$ and $\failure_2$ are not \factive, it is possible for $\test_1$ to return $0$ outcome.
Conversely, in the fifth row, it says that it not possible for $\test_1$ to return \fail~($1$) if both \fmodes~in its scope are \finactive.
For example suppose that $\test_1$ fails, $\tfactor_1$ says that the possible states for $(\failure_1, \failure_2)$ are $(0,1)$, $(1,0)$ and $(1,1)$.
Similarly, $\tfactor_2$ says that the possible states for $(\failure_2, \failure_3)$ are $(0,0)$, $(1,1)$.
Joining the possible states we get that the possible states for $(\failure_1, \failure_2, \failure_3)$ are $(0,1,1)$, $(1,0,0)$, $(1,1,1)$.
Without additional information, we cannot say which of the possible states is the correct one.
We will study this phenomenon in~\cref{sec:foundamental_limits}.

\myParagraph{Probabilistic}
As we pointed out earlier, deterministic tests are not easy to implement.
For this reason, in this paper, we also allow for an arbitrary probabilistic relationship between test outcomes and \fmodes~in test scopes.
For the sake of simplicity, we will discuss tests that we call \emph{well behaved} (similar to the one used in~\cite{abdollahi2016book-pgmFaultDiagnosis}).
We call a \dtest~well behaved if 
\begin{equation}
  \Pr(\syndromevar\mid\faultsover{\scope(\test)}) = \prod_{\failure_i\in\scope(\test)} \Pr(\syndromevar\mid\failure_i)
\end{equation}
Now suppose each test has a probability $p_{d,i}$ of correctly identify failure $\failure_i$ (detection probability), and a probability $p_{f,i}$ of false alarm for $\failure_i$, as illustrated in \cref{fig:well_behaved_tests}.
Exploiting the fact that $\failure_i\in\{0,1\}$, we can write
% \begin{align*}
%   \Pr(\test=\textrm{\pass}\mid\faultsover{\scope(\test)}) &= \prod_{\failure_i\in\scope(\test)} \Pr(\test=\textrm{\pass}\mid\failure_i) = (1-p_{d,i})^{\failure_i} (1-p_{f,i})^{1-\failure_i} \\
%   \Pr(\test=\textrm{\fail}\mid\faultsover{\scope(\test)}) &= \prod_{\failure_i\in\scope(\test)} \Pr(\test=\textrm{\fail}\mid\failure_i) = (p_{d,i})^{\failure_i} (p_{f,i})^{1-\failure_i}
% \end{align*}
\begin{equation*}
  \Pr(\syndromevar\mid\failure_i) =
  \begin{cases}
    (1-p_{d,i})^{\failure_i} (1-p_{f,i})^{1-\failure_i} &\text{if~}\,\test=\textrm{\pass}  \\
    (p_{d,i})^{\failure_i} (p_{f,i})^{1-\failure_i} &\text{if~}\, \test=\textrm{\fail}  \\
  \end{cases}
\end{equation*}
The potentials for the factor $\tfactor_1$ in \cref{fig:simple_dgraph} are reported in the column `Well behaved test' in \cref{tab:tfactor_1}.
Notice that perfect tests are not well behaved.
In fact from from the last row we need $p_{d,1}=p_{d,2}=1$, substituting in the forth row we get $\Pr(\test=\textrm{\pass}\mid \failure_1,\failure_2=\textrm{\factive}) = 0 \neq 1$, thus violating the third condition in \cref{eq:perfect_test}.

Let again fail $\test_1$.
Pick $p_{d,i} = 0.95$ and $p_{f,i}=0.1$ for all $i=1,2,3$.
By multiplying the two factors and normalizing, we get that the most probable state for $(\failure_1, \failure_2, \failure_3)$ is $(1,0,0)$ with probability $0.56$.
% Of course different choices of detection and false alarm probabilities would lead to different results.

In arbitrary probabilistic tests, we could have any value in the table.
It is worth noticing that the expressive power of the factor graph allows us to put any value in the factor table, and we are not restricted to probabilities.

\begin{figure}[!ht]
  \centering
  \includestandalone{figures/well_behaved_tests}
  \caption{Relation between test outcome and \fmodes~state in well behaved tests~\cite{abdollahi2016book-pgmFaultDiagnosis}.}
  \label{fig:well_behaved_tests}
\end{figure}

\begin{table}[!ht]
  \centering\begin{tabular}{c|c|c||c||l}
    $\syndromevar_1$ & $\failure_1$ & $\failure_2$ & Perfect test & Well behaved test \\
    \hline
    0 & 0 & 0 & 1 & $(1 - p_{f,1}) (1 - p_{f,2})$\\
    0 & 0 & 1 & 0 & $(1 - p_{f,1}) (1 - p_{d,2})$\\
    0 & 1 & 0 & 0 & $(1 - p_{d,1}) (1 - p_{f,2})$\\
    0 & 1 & 1 & 1 & $(1 - p_{d,1}) (1 - p_{d,2})$\\
    1 & 0 & 0 & 0 & $(p_{f,1})(p_{f,2})$\\
    1 & 0 & 1 & 1 & $(p_{f,1})(p_{d,2})$\\
    1 & 1 & 0 & 1 & $(p_{d,1})(p_{f,2})$\\
    1 & 1 & 1 & 1 & $(p_{d,1})(p_{d,2})$\\
  \end{tabular}
  \caption{Table associated to a factor for a perfect or well behaved test.}
  \label{tab:tfactor_1}
\end{table}



==> sections/subsections/training.tex <==
%!TEX root = ../../main.tex

% \subsection{Parameters Learning}

% In this section we will describe how to learn the supervised learning for factor graphs and graph neural networks.



==> tables/fault_identification_alt_both.tex <==
\begin{table}
  % \hspace*{-2cm}
  \smaller
  \begin{tabular}{ |l||c|c|c|c|c|c| }
    \hline
    \multirow{2}{*}{\textbf{Algorithm}} & \multicolumn{3}{c|}{\textbf{Regular}} & \multicolumn{3}{c|}{\textbf{Temporal}}\\
    & All & Outputs & Modules & All & Outputs & Modules \\    \hline
    GCN        & 91.33       & 95.45         & 78.94        & 88.42       & 92.08       & 77.45 \\
    GCNII      & \fst{92.80} & \fst{96.41}   & \fst{81.97}  & 92.33 & \fst{96.57}       & 79.60 \\
    GIN        & \fst{92.65} & \fst{96.77}   & \fst{80.30}  & 88.42       & 92.08       & 77.45 \\
    GraphSage  & 90.08       & 93.94         & 78.48        & 91.10       & 94.84       & 79.91 \\
   \hline
  \end{tabular}
  \caption{Accuracy ablation study for fault identification with alternative \fmode and test features.}
  \label{tab:fault_identification_alt_fmodes}
\end{table}

==> tables/fault_identification_alt_fmodes.tex <==
\begin{table}
  % \hspace*{-2cm}
  \smaller
  \begin{tabular}{ |l||c|c|c|c|c|c| }
    \hline
    \multirow{2}{*}{\textbf{Algorithm}} & \multicolumn{3}{c|}{\textbf{Regular}} & \multicolumn{3}{c|}{\textbf{Temporal}}\\
    & All & Outputs & Modules & All & Outputs & Modules \\    \hline
    GCN        & 91.40       & 95.20       & 80.00       & 90.80       & 94.73       & 78.99 \\
    GCNII      & \fst{90.83} & \fst{94.95} & \fst{78.48} & \fst{89.92} & 94.07       & 77.45 \\
    GIN        & \fst{93.07} & \fst{96.67} & 82.27       & 88.88       & 92.48       & 78.07 \\
    GraphSage  & \fst{93.30} & \fst{96.67} & \fst{83.18} & 92.25       & 95.76       & \fst{81.75} \\
   \hline
  \end{tabular}
  \caption{Accuracy ablation study for fault identification with alternative \fmode features.}
  \label{tab:fault_identification_alt_fmodes}
\end{table}

==> tables/fault_identification_alt_tests.tex <==
\begin{table}
  % \hspace*{-2cm}
  \smaller
  \begin{tabular}{ |l||c|c|c|c|c|c| }
    \hline
    \multirow{2}{*}{\textbf{Algorithm}} & \multicolumn{3}{c|}{\textbf{Regular}} & \multicolumn{3}{c|}{\textbf{Temporal}}\\
    & All & Outputs & Modules & All & Outputs & Modules \\    \hline
    GCN        & 91.40       & 95.45       & 79.24       & 91.41       & 95.09       & \fst{80.37} \\
    GCNII      & \fst{93.07} & \fst{96.57} & \fst{82.58} & \fst{92.71} & 96.06 & \fst{82.67} \\
    GIN        & 89.09       & 92.63       & 78.48       & 88.42       & 92.08       & 77.45 \\
    GraphSage  & \fst{93.07} & \fst{96.62} & 82.42       & 91.18       & 94.58       & 80.98 \\
   \hline
  \end{tabular}
  \caption{Accuracy ablation study for fault identification with alternative test features.}
  \label{tab:fault_identification_alt_tests}
\end{table}

==> tables/scenarios.tex <==
\begin{longtable}{ l l p{6cm} }
  \caption{Scenarios}\label{tab:scenarios}\\
  \textbf{Name} & \textbf{Map} & \textbf{Description} \\
  \hline
  Overturned Truck & Borregas Avenue & 
  The ego vehicle is driving down a straight road that is occupied by an overturned truck.
  The scenario recreates an incident occurred in Taiwan where a Tesla hit an overturned truck on an highway.
  \\
  Stopped Vehicle & Borregas Avenue & 
  While driving, the car in front of the ego vehicle makes a lane change to avoid the stationary car that is in their lane. 
  This leaves the ego vehicle with little to no time to react to this stationary car.
  \\
  Invisible Pedestrian & Borregas Avenue &
  While driving through a street that has a truck parked on the right side, a pedestrian steps into the road from directly behind the parked truck.
  \\
  Cut Off Left & Borregas Avenue &
  While driving in the right lane of a three lane road, an agent from the left lane cuts the ego vehicle off.
  \\
  Cut Off Right & Borregas Avenue &
  While driving in the left lane of a two lane road, an agent from the right lane cuts the ego vehicle off while turning into a parking lot.
  \\
  School Bus Intersection & Borregas Avenue &
  The ego vehicle drives through an intersection that includes a school bus driving in front it coming from the edge of the field of view.
  As the ego vehicle crosses the intersection, a pedestrian steps into the intersection from the left side.
  \\
  Cones in the Lane & Borregas Avenue &
  The ego vehicle is driving in a lane with traffic cones to the right while an agent is driving in the opposite direction on the left. 
  After the traffic cones have been passed, an agent pulls oit of a parking lot right in front of the ego vehicle.
  \\ 
  Cyclist & Borregas Avenue &
  The ego vehicle starts in front of an intersection and once it begins driving, a cyclist enters the field of view from the left side of the intersection and rides right in front of the ego vehicle.
  \\
  Turkeys & GoMentum &
  While driving on a straight road, the ego vehicle must avoid a collision with two turkeys that walk into the road.
  \\ 
  Unprotected Right Turn & GoMentum &
  The ego vehicle makes an unprotected right turn on a road that contains an agent driving down it as well as another right turn about 20 yards to the left of the ego vehicle that has an agent waiting to exit.
\end{longtable}

==> tables/scenarios_ext.tex <==
%!TEX root = ../main.tex

\setlength\LTleft{-2cm}
\begin{longtable}{ p{5cm} p{5cm} p{5cm} }
  \caption{Scenarios}\label{tab:scenarios}\\
  \textbf{Context} & \textbf{Scene} & \textbf{Example} \\
  % \hline\noalign{\vskip 0.5cm}
  \midrule %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \raisebox{10pt}{\includegraphics[width=5cm]{figures/scenarios/invisible_pedestrian_scene.jpg}}
  &
  \includegraphics[width=5cm]{figures/scenarios/invisible_pedestrian.png}
  &
  \begin{tikzpicture}[
    path image/.style={path picture={
      \node at (1,3) {\includegraphics[scale=0.8, rotate=105]{figures/scenarios/invisible_pedestrian.pdf}};}
    }]
    \path [path image] (0,0) rectangle (\linewidth, 3cm);
  \end{tikzpicture}
  \\
  \multicolumn{3}{p{16cm}}{
    \textbf{Invisible Pedestrian}.
    While driving through a street that has a truck parked on the right side, a pedestrian steps into the road from directly behind the parked truck.
  }\\
  \midrule %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \raisebox{10pt}{\includegraphics[width=5cm]{figures/scenarios/overturned_truck.jpg}}
  &
  \includegraphics[width=5cm]{figures/scenarios/overturned_truck.png}
  &
  \begin{tikzpicture}[
    path image/.style={path picture={
      \node at (2.2,3) {\includegraphics[scale=0.4, rotate=105]{figures/scenarios/overturned_truck.pdf}};}
    }]
    \path [path image] (0,0) rectangle (\linewidth, 3cm);
  \end{tikzpicture}
  \\
  \multicolumn{3}{p{16cm}}{
    \textbf{Overturned Truck}.
    The ego vehicle is driving down a straight road that is occupied by an overturned truck.
    The scenario recreates an incident occurred in Taiwan where a Tesla hit an overturned truck on an highway.
  }\\
  \midrule %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \raisebox{10pt}{\includegraphics[width=5cm]{figures/scenarios/stopped_vehicle_curved.jpg}}
  &
  \includegraphics[width=5cm]{figures/scenarios/stopped_vehicle_curved.png}
  &
  \begin{tikzpicture}[
    path image/.style={path picture={
      \node at (-1,3) {\includegraphics[scale=0.8, rotate=105]{figures/scenarios/stopped_vehicle_curved.pdf}};}
    }]
    \path [path image] (0,0) rectangle (\linewidth, 3cm);
  \end{tikzpicture}
  \\
  \multicolumn{3}{p{16cm}}{
    \textbf{Stopped Vehicle}.
    While driving, the car in front of the ego vehicle makes a lane change to avoid the stationary car that is in their lane. 
    This leaves the ego vehicle with little to no time to react to this stationary car.
  }\\
  \midrule %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \raisebox{10pt}{\includegraphics[width=5cm]{figures/scenarios/cut_off_left.jpg}}
  &
  \includegraphics[width=5cm]{figures/scenarios/cut_off_left.png}
  &
  \begin{tikzpicture}[
    path image/.style={path picture={
      \node at (6.2,4) {\includegraphics[scale=0.8, rotate=105]{figures/scenarios/cut_off_left.pdf}};}
    }]
    \path [path image] (0,0) rectangle (\linewidth, 3cm);
  \end{tikzpicture}
  \\
  \multicolumn{3}{p{16cm}}{
    \textbf{Cut Off Left}.
    While driving in the right lane of a three lane road, an agent from the left lane cuts the ego vehicle off.
  }\\
  \midrule %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \raisebox{10pt}{\includegraphics[width=5cm]{figures/scenarios/cut_off_right.jpg}}
  &
  \includegraphics[width=5cm]{figures/scenarios/cut_off_right.png}
  &
  \begin{tikzpicture}[
    path image/.style={path picture={
      \node at (6.5,4) {\includegraphics[scale=0.8, rotate=105]{figures/scenarios/cut_off_right.pdf}};}
    }]
    \path [path image] (0,0) rectangle (\linewidth, 3cm);
  \end{tikzpicture}
  \\
  \multicolumn{3}{p{16cm}}{
    \textbf{Cut Off Right}.
    While driving in the left lane of a two lane road, an agent from the right lane cuts the ego vehicle off while turning into a parking lot.
  }\\
  \midrule %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \raisebox{10pt}{\includegraphics[width=5cm]{figures/scenarios/school_bus_intersection.jpg}}
  &
  \includegraphics[width=5cm]{figures/scenarios/school_bus_intersection.png}
  &
  \begin{tikzpicture}[
    path image/.style={path picture={
      \node at (6.5,4) {\includegraphics[scale=0.8, rotate=105]{figures/scenarios/school_bus_intersection.pdf}};}
    }]
    \path [path image] (0,0) rectangle (\linewidth, 3cm);
  \end{tikzpicture}
  \\
  \multicolumn{3}{p{16cm}}{
    \textbf{School Bus Intersection}.
    The ego vehicle drives through an intersection that includes a school bus driving in front it coming from the edge of the field of view.
    As the ego vehicle crosses the intersection, a pedestrian steps into the intersection from the left side.
  }\\
  \midrule %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \raisebox{10pt}{\includegraphics[width=5cm]{figures/scenarios/traffic_cones_complex.jpg}}
  &
  \includegraphics[width=5cm]{figures/scenarios/traffic_cones_complex.png}
  &
  \begin{tikzpicture}[
    path image/.style={path picture={
      \node at (4.5,3) {\includegraphics[scale=0.8, rotate=105]{figures/scenarios/traffic_cones_complex.pdf}};}
    }]
    \path [path image] (0,0) rectangle (\linewidth, 3cm);
  \end{tikzpicture}
  \\
  \multicolumn{3}{p{16cm}}{
    \textbf{Cones in the Lane}.
    The ego vehicle is driving in a lane with traffic cones to the right while an agent is driving in the opposite direction on the left. 
    After the traffic cones have been passed, an agent pulls oit of a parking lot right in front of the ego vehicle.
  }\\
  \midrule %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \raisebox{10pt}{\includegraphics[width=5cm]{figures/scenarios/cyclist.jpg}}
  &
  \includegraphics[width=5cm]{figures/scenarios/cyclist.png}
  &
  \begin{tikzpicture}[
    path image/.style={path picture={
      \node at (9,3) {\includegraphics[scale=1.2, rotate=105]{figures/scenarios/cyclist.pdf}};}
    }]
    \path [path image] (0,0) rectangle (\linewidth, 3cm);
  \end{tikzpicture}
  \\
  \multicolumn{3}{p{16cm}}{
    \textbf{Cyclist}.
    The ego vehicle starts in front of an intersection and once it begins driving, a cyclist enters the field of view from the left side of the intersection and rides right in front of the ego vehicle.
  }\\
  \midrule %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \raisebox{10pt}{\includegraphics[width=5cm]{figures/scenarios/turkeys.jpg}}
  &
  \includegraphics[width=5cm]{figures/scenarios/turkeys.png}
  &
  \begin{tikzpicture}[
    path image/.style={path picture={
      \node at (-4,1) {\includegraphics[scale=0.8, rotate=28]{figures/scenarios/turkeys.pdf}};}
    }]
    \path [path image] (0,0) rectangle (\linewidth, 3cm);
  \end{tikzpicture}
  \\
  \multicolumn{3}{p{16cm}}{
    \textbf{Turkeys}.
    While driving on a straight road, the ego vehicle must avoid a collision with two turkeys that walk into the road.
  }
\end{longtable}


% \begin{table}[ht]
%   \caption{A table arranging  images}
%   \centering
%   \begin{tabular}{cc}
%   \includegraphics[width=4cm]{figures/scenarios/invisible_pedestrian_scene.jpg}&
%   \includegraphics[width=4cm]{figures/scenarios/invisible_pedestrian.png}\\
   
%   \end{tabular}
%   \label{tab:gt}
%   \end{table}
